OpenGraph: Towards Open Graph Foundation Models

Graph learning has become essential in various domains, including recommendation systems and social network analysis. Graph Neural Networks (GNNs) have emerged as promising techniques for encoding structural information and improving performance in tasks like link prediction and node classification. However, a key challenge remains: the difficulty of generalizing to unseen graph data with different properties. In this work, we propose a novel graph foundation model, called OpenGraph, to address this challenge. Our approach tackles several technical obstacles. Firstly, we enhance data augmentation using a large language model (LLM) to overcome data scarcity in real-world scenarios. Secondly, we introduce a unified graph tokenizer that enables the model to generalize effectively to diverse graph data, even when encountering unseen properties during training. Thirdly, our developed scalable graph transformer captures node-wise dependencies within the global topological context. Extensive experiments validate the effectiveness of our framework. By adapting OpenGraph to new graph characteristics and comprehending diverse graphs, our approach achieves remarkable zero-shot graph learning performance across various settings. We release the model implementation at https://github.com/HKUDS/OpenGraph.

==> tem.tex <==

\begin{table*}[t]
    \centering
    \caption{Performance comparison between our \model\ (zero-shot) and baseline methods (one-shot, five-shot) on the link prediction task (measured by \textit{Recall@N} for $N=20, 40$) and node classification task (measured by \textit{Accuracy} and \textit{Macro F1 Score}).}
    \label{tab:overall_performance}
    % \small
    % \footnotesize
    \scriptsize
    \setlength{\tabcolsep}{.9mm}
    \vspace{-.15in}
    % \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    % \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c||c|c|c|c|c|c}
        \hline
        \multicolumn{2}{c|}{Dataset} & \multicolumn{2}{c|}{ogbl-ddi} & \multicolumn{2}{c|}{ogbl-collab} & \multicolumn{2}{c|}{ML-1M} & \multicolumn{2}{c|}{ML-10M} & \multicolumn{2}{c||}{Amazon-book} & \multicolumn{2}{c|}{Cora} & \multicolumn{2}{c|}{Citeseer} & \multicolumn{2}{c}{Pubmed}\\
        \hline
        Model & shot & R@20 & R@40 & R@20 & R@40& R@20 & R@40& R@20 & R@40& R@20 & R@40 & Acc & MacF1 & Acc & MacF1 & Acc & MacF1\\
        \hline
        \hline
        \multirow{2}{*}{MF} & 1 & .0087 & .0161 & .0261 & .0349 & .0331 & .0604 & .1396 & .1956 & .0034 & .0043 & .1710 & .1563 & .1740 & 	.1727 & .3470 &  .3346\\
        \cline{2-18}
        & 5 & .0536 & .0884 & .0412 & .0609 & .0987 & .1584 & .2060 & .2989 & .0196 & .0284 & .1500 & .1422 & .1520 & .1484 & .3540 & .3435\\
        \hline
        \multirow{2}{*}{MLP} & 1 & .0195 & .0336 & .0112 & .0185 & .0548 & .1019 & .1492 & .2048 & .0017 & .0028 & .2300 & .1100 & .2590 & .1993 & .4430 & .3114\\
        \cline{2-18}
        & 5 & .0621 & .1038 & .0115 & .0185 & .0851 & .1470 & .2362 & .2563 & .0092 & .0152 & .3930 & .3367 & .3690 & .3032 & .5240 & .4767\\
        \hline
        \multirow{2}{*}{GCN} & 1 & .0279 & .0459 & .0206 & .0321 & .0432 & .0849 & .1760 & .2086 & .0096 & .0160 & .3180 & .1643 & .3200 & .2096 & .4270 & .3296\\
        \cline{2-18}
        & 5 & .0705 & .1312 & .0366 & .0513 & .1054 & .1656 & .2127 & .2324 & .0251 & .0408 & .5470 & .5008 & .4910 & .4190 & .509 & .4455\\
        \hline
        \multirow{2}{*}{GAT} & 1 & .0580 & .1061 & .0258 & .0372 & .0245 & .0520 & .1615 & .2476 & .0047 & .0079 & .2420 & .1687 & .2810 & .2025 & .4720	& .3657\\
        \cline{2-18}
        & 5 & .0711 & .1309 & .0340 & .0505 & .1506 & .2267 & .2002 & .2883 & .0228 & .0392 & .585 & .5438 & .4940 & .4441 & .5780 & .5582\\
        \hline
        \multirow{2}{*}{GIN} & 1 & .0530 & .1004 & .0163 & .0247 & .0466 & .0884 & .1541 & .2388 & .0069 & .0114 & .3190 & .1753 & .2820 & .1705 & .4410 & .3064\\
        \cline{2-18}
        & 5 & .0735 & .1441 & .0311 & .0458 & .1458 & .2344 & .1926 & .2829 & .0252 & .0418 & .5400 & .4941 & .521 & .4696 & .5070 & .4547\\
        \hline
        \multirow{2}{*}{DGI} & 1 & .0315 & .0617 & .0255 & .0385 & .0486 & .0863 & .1868 & .2716 & .0081 & .0142 & .3150 & .1782 & .2840 & .1791 & .4290 & .3163\\
        \cline{2-18}
        & 5 & .0821 & .1426 & .0345 & .0502 & .1687 & .2573 & .2303 & .3063 & .0300 & .0492 & .4880 & .4606 & .4450 & .4062 & .4890 & .4509\\
        \hline
        \multirow{2}{*}{GPF} & 1 & .0503 & .0856 & .0027 & .0048 & .1099 & .1702 & .1599 & .2326 & .0072 & .0128 & .3080 & .1952 & .3110 & .1984 & .4220 & .2670\\
        \cline{2-18}
        & 5 & .0839 & .1460 & .0027 & .0047 & .0817 & .1392 & .2014 & .2994 & .0179 & .0310 & .5550 & .5233 & .4690 & .4223 & .5150 & .4934\\
        \hline
        \multirow{2}{*}{GPrompt} & 1 & .0541 & .1102 & .0138 & .0207 & .0797 & .1310 & .1362 & .2073 & .0074 & .0120 & .3540 & .1596 & .2800 & .1519 & .4710 & .3705\\
        \cline{2-18}
        & 5 & .0769 & .1396 & .0157 & .0231 & .1340 & .2166 & .2157 & .3147 & .0287 & .0464 & .5510 & .5098 & .5570 & .5211 & .5130 & .4520\\
        \hline
        \multirow{2}{*}{GraphCL} & 1 & .0603 & .1112 & .0265 & .0398 & .0390 & .0799 & .1655 & .2529 & .0047 & .0077 & .2430 & .1548 & .2980 & .1630 & .4070 & .4130\\
        \cline{2-18}
        & 5 & .0740 & .1368 & .0311 & .0456 & .1416 & .2138 & .2019 & .3075 & .0270 & .0440 & .5610 & .5330 & .4300 & .3683 & .5230 & .5024\\
        \hline
        % \hline
        % GPT-3.5 & 0-shot\\
        % \hline
        % GPT-4 & 0-shot\\
        \hline
        Ours & 0 & \textbf{.0921} & \textbf{.1746} & \textbf{.0421} & \textbf{.0639} & \textbf{.1911} & \textbf{.2978} & \textbf{.2370} & \textbf{.3265} & \textbf{.0485} & \textbf{.0748} & \textbf{.7504} & \textbf{.7426} & \textbf{.6097} & \textbf{.5821} & \textbf{.6869} & \textbf{.6537}\\
        \hline
    \end{tabular}
    \vspace{-.05in}
\end{table*}


ogbl-ddi & .0737 & \underline{.0893} & .0656 & .0588 & .0770 & .0692 & \textbf{.0921}\\
        \hline
        ML1M & .0572 & .1680 & .0850 & .0599 & .0485 & \textbf{.2030} & \underline{.1911}\\
        \hline
        ML10M & .0982 & .1636 & .1017 & .1629 & .0910 & \textbf{.2698} & \underline{.2370}\\
        \hline
        Cora & .4985 & .4864 & .4342 & .3715 & \underline{.5943} & .2780 & \textbf{.7504}\\
        \hline
        Citeseer & .3944 & .3691 & \underline{.5743} & .2651 & .4300 & .2003 & \textbf{.6097}\\
        \hline
        Pubmed & .4501 & .5015 & .4876 & .3317 & \underline{.5148} & .3652 & \textbf{.6869}\\
        \hline
